TableLlama: Towards Open Large Generalist Models for Tables

Semi-structured tables are ubiquitous. There has been a variety of tasks that aim to automatically interpret, augment, and query tables. Current methods often require pretraining on tables or special model architecture design, are restricted to specific table types, or have simplifying assumptions about tables and tasks. This paper makes the first step towards developing open-source large language models (LLMs) as generalists for a diversity of table-based tasks. Towards that end, we construct TableInstruct, a new dataset with a variety of realistic tables and tasks, for instruction tuning and evaluating LLMs. We further develop the first open-source generalist model for tables, TableLlama, by fine-tuning Llama 2 (7B) with LongLoRA to address the long context challenge. We experiment under both in-domain setting and out-of-domain setting. On 7 out of 8 in-domain tasks, TableLlama achieves comparable or better performance than the SOTA for each task, despite the latter often has task-specific design. On 6 out-of-domain datasets, it achieves 5-44 absolute point gains compared with the base model, showing that training on TableInstruct enhances the model's generalizability. We open-source our dataset and trained model to boost future work on developing open generalist models for tables.

==> abstract.tex <==
\begin{abstract}

As large language models (LLMs) are excellent assistants to communicate with humans, the problem of enabling large language models to effectively understand tables and complete table-related tasks is a crucial step in facilitating human-machine interactions, which can provide a convenient unified interface to assist humans handling table tasks. Towards this end, we introduce \texttt{TableBench}, a comprehensive table benchmark which integrates different table types and table tasks from different real-world scenarios and construct 968k instruction tuning dataset. Based on \texttt{TableBench}, we conduct an initial exploration of using LLMs for building generalist table models. During the unification of different table tasks, we encounter three main challenges due to the input length limit of LLMs: large table input, large category classification and large candidate ranking. We propose three algorithms: dynamic subtable segmentation, divide-and-merge and tree-rank to resolve them respectively. Our experiments show that: with only no more than 1.4\% training data, LLMs can achieve more than 60\% SOTA performance on most table tasks; with 5\%-40\% training data, LLMs can achieve more than 80\% SOTA performance on most table tasks, and some can even be better than SOTA.\footnote{Our dataset, code and models will be available.}


% Dynamic subtable segmentation reserves different lengths for different components of instructions for different tasks and calculates the allowed subtable length and segments table accordingly. Divide-and-merge first divides entire large categories into different subsets and each subset is formulated as the candidates in a multi-choice QA problem for the model to select the correct candidate, then merges the answer from all the subsets. Tree-rank ranks entire candidates by multiple node splitting and merging processes, which prioritizes merging the top-ranked half node pairs each time.












% The abstract paragraph should be indented 1/2~inch (3~picas) on both left and
% right-hand margins. Use 10~point type, with a vertical spacing of 11~points.
% The word \textsc{Abstract} must be centered, in small caps, and in point size 12. Two
% line spaces precede the abstract. The abstract must be limited to one
% paragraph.

% Our solution demonstrates a decent level of performance, but there is still substantial room to improve for some tasks to compete with the state-of-the-art customized models with special model architecture design or table pretraining. 

\end{abstract}

==> abstract2.tex <==
\begin{abstract}

As large language models (LLMs) are excellent assistants to communicate with humans, the problem of enabling large language models to effectively understand tables and complete table-related tasks is a crucial step in facilitating human-machine interactions, which can provide a convenient unified interface to assist humans handling table tasks. Towards this end, we introduce \texttt{TableBench}, a comprehensive table benchmark which integrates different table types and table tasks from different real-world scenarios and construct 968k instruction tuning dataset. Based on \texttt{TableBench}, we conduct an initial exploration of using LLMs for building generalist table models. During the unification of different table tasks, we encounter three main challenges due to the input length limit of LLMs: large table input, large category classification and large candidate ranking. We propose three algorithms: dynamic subtable segmentation, divide-and-merge and tree-rank to resolve them respectively. Our experiments show that: with only no more than 1.4\% training data, LLMs can achieve more than 60\% SOTA performance on most table tasks; with 5\%-40\% training data, LLMs can achieve more than 80\% SOTA performance on most table tasks, and some can even be better than SOTA.\footnote{Our dataset, code and models will be available.}


% Dynamic subtable segmentation reserves different lengths for different components of instructions for different tasks and calculates the allowed subtable length and segments table accordingly. Divide-and-merge first divides entire large categories into different subsets and each subset is formulated as the candidates in a multi-choice QA problem for the model to select the correct candidate, then merges the answer from all the subsets. Tree-rank ranks entire candidates by multiple node splitting and merging processes, which prioritizes merging the top-ranked half node pairs each time.












% The abstract paragraph should be indented 1/2~inch (3~picas) on both left and
% right-hand margins. Use 10~point type, with a vertical spacing of 11~points.
% The word \textsc{Abstract} must be centered, in small caps, and in point size 12. Two
% line spaces precede the abstract. The abstract must be limited to one
% paragraph.

% Our solution demonstrates a decent level of performance, but there is still substantial room to improve for some tasks to compete with the state-of-the-art customized models with special model architecture design or table pretraining. 

\end{abstract}

==> algorithms/algo1.tex <==
\begin{algorithm}[!htbp]
\caption{Pseudo code of Dynamic Subtable Segmentation}
\label{algo1}
\KwIn{Segmented subtable set: $sub\_tab\_set = \emptyset$. $input$ contains prompt, table metadata, $table$ and instruction. Initialize the maximum input length: $L_{max}$, reserved prompt length: $L_{pro}$, reserved instruction length: $L_{ins}$, reserved table metadata length: $L_{meta}$ for each task and the offset. Denote input length as $L_{inp}$ and serialized table length as $L_{tab}$. Note all lengths here refer to the length after tokenization, rather than the original string length.}
\KwOut{the final subtable set $S$.}
$L_{inp} = L_{pro} + L_{meta} + L_{tab} + L_{ins}$ \\
\If{$L_{inp} > L_{max}$}
{
$seg\_tab\_num = \lceil L_{tab} / (L_{max} - L_{pro} - L_{ins} - L_{meta} - $ offset$) \rceil$ TO EXPLAIN THIS \\
\For{$i\in1,2, ..., seg\_tab\_num$}
{
\If{$i=1$}
{
$start\_idx = 0$ \\
$end\_idx = L_{max} - L_{ins} - L_{pro} - L_{meta}$ \\
}
\Else
{
$start\_idx = end\_idx - $ offset \\
$end\_idx = start\_idx + L_{max} - L_{ins} - L_{pro} - L_{meta}$\\
}
$sub\_table\_set = sub\_table\_set \cup table[start\_idx: end\_idx]$ \\
}   
}
\Else
{
$sub\_table\_set = input$ \\
}
return $sub\_table\_set$
\end{algorithm}


==> algorithms/algo2.tex <==
\begin{algorithm}[H]
\caption{Pseudo code of Divide and Merge}
\label{algo2}
\KwIn{Initialize the set size: $s$.}
\KwOut{the final prediction $\mathcal{P}$.}

\textbf{Divide (training \& inference):} \\
\qquad Divide the entire candidate set $\displaystyle \sA$ into different subsets: $\displaystyle \sA_i$ according to the set size $s$. \\
\qquad For each subset $\displaystyle \sA_i$, add "none of the above" and randomly shuffle it. \\
\qquad Let the model choose correct answers from each subset $\displaystyle \sA_i$.\\

\textbf{Merge (inference):} \\
\qquad Merge all the predictions from all the subsets as the final prediction. \\
\qquad Merge all the ground truths from all the subsets as the final ground truth. \\
\qquad Remove the "none of the above" from both prediction and ground truth. \\ 

\textbf{Return prediction $\mathcal{P}$.}
\end{algorithm}


==> algorithms/algo3.tex <==
\begin{algorithm}[H]
\caption{Pseudo code of Tree Rank (for each sublayer)}
\label{algo3}
\KwIn{Subsets needed to be ranked: $\{\displaystyle \sA_1, \displaystyle \sA_2,... \displaystyle \sA_n\}$. Optional: single half $H^f$ and $H^b$ from last layer.}
\KwOut{The merged front halves $\{\displaystyle \sA^f_1, \displaystyle \sA^f_2,... \displaystyle \sA^f_{n/2}\}$ and the merged bottom halves $\{\displaystyle \sA^b_1, \displaystyle \sA^b_2,... \displaystyle \sA^b_{n/2}\}$. Optional: the last subset half $H^f_n$ and $H^b_n$.}
{
% Reinitialize the number of the subset $n$. \\
Let the model rank each subset $\displaystyle \sA_i$. \\
Divide elements of each ranked subset into two halves based on the order: the front half $H^f_i$ and the bottom half $H^b_i$, $i\in \{1,2,...,n\}$. \\
\If{$n\%2 == 0$}
{
Merge all the front halves $H^f_i$ in pairs and get the new subsets: $\displaystyle \sA^f_k$, $\displaystyle \sA^f_k = H^f_i\cup H^f_{i+1}$. \\ 
Merge all the bottom halves $H^b_i$ in pairs and get the new subsets: $\displaystyle \sA^b_k$, $\displaystyle \sA^b_k = H^b_i\cup H^b_{i+1}$. \\ 
Get all the merged front halves $\{\displaystyle \sA^f_1, \displaystyle \sA^f_2,... \displaystyle \sA^f_{n/2}\}$
and all the merged bottom halves $\{\displaystyle \sA^b_1, \displaystyle \sA^b_2,... \displaystyle \sA^b_{n/2}\}$.
}
\Else{
Merge all the front halves $H^f_i$ in pairs and get the new subsets: $\displaystyle \sA^f_k$ except the last half $H^f_n$. \\ 
Merge all the bottom halves $H^b_i$ in pairs and get the new subsets: $\displaystyle \sA^b_k$ except the last half $H^b_n$.\\ 
Get all the merged front halves $\{\displaystyle \sA^f_1, \displaystyle \sA^f_2,... \displaystyle \sA^f_{(n-1)/2}\}$ and all the merged bottom halves $\{\displaystyle \sA^b_1, \displaystyle \sA^b_2,... \displaystyle \sA^b_{(n-1)/2}\}$. \\
\If{
$H^f$ exists and $H^b$ exists
}
{
Merge $H^f$ and $H^f_n$ to be $\displaystyle \sA^f_{n/2}$. Merge $H^b$ and $H^b_n$ to be $\displaystyle \sA^b_{n/2}$. 
}
\Else{
Convey the last subset half $H^f_n$ and $H^b_n$ to the next layer. 
}
}
Make sure all the merged front halves $\{\displaystyle \sA^f_1, \displaystyle \sA^f_2,... \displaystyle \sA^f_{n/2}\}$
are in front of all the merged bottom halves $\{\displaystyle \sA^b_1, \displaystyle \sA^b_2,... \displaystyle \sA^b_{n/2}\}$.
}

\end{algorithm}


% \begin{algorithm}[H]
% \caption{Pseudo code of Tree Rank}
% \label{algo3}
% \KwIn{Initialize the set size: $s$, the list needed to be ranked: $L_S$.}
% \KwOut{the final ranked list $L_R$.}
% $n = |L_S| / s$, randomly shuffle $L_S$ and divide $L_S$ to $n$ subsets $\displaystyle \sA_i$, where $i\in \{1,2,...,n\}$. \\
% \SetKwFunction{FMain}{\textbf{TreeRank}}
% \SetKwProg{Fn}{Def}{:}{}
% \Fn{\FMain{$\displaystyle \sA_1, \sA_2,...\sA_n$}}{
% Reinitialize the number of the subset $n$. Let the model rank each subset. \\
% Divide elements of each ranked subset into two halves based on the order: the front half $H^f_i$ and the bottom half $H^b_i$, $i\in \{1,2,...,n\}$. \\
% \If{$n\%2 == 0$}
% {
% Merge all the front halves $H^f_i$ in pairs and get the new subsets: $\displaystyle \sA^f_k$, $\displaystyle \sA^f_k = H^f_i\cup H^f_{i+1}$. \\ 
% Merge all the bottom halves $H^b_i$ in pairs and get the new subsets: $\displaystyle \sA^b_k$, $\displaystyle \sA^b_k = H^b_i\cup H^b_{i+1}$. \\ 
% Return all the merged front halves $\{\displaystyle \sA^f_1, \displaystyle \sA^f_2,... \displaystyle \sA^f_{n/2}\}$
% and all the merged bottom halves $\{\displaystyle \sA^b_1, \displaystyle \sA^b_2,... \displaystyle \sA^b_{n/2}\}$. \\
% }
% \Else{
% Merge all the front halves $H^f_i$ in pairs and get the new subsets: $\displaystyle \sA^f_k$ except for the last half $H^f_n$. 
% \\ Merge all the bottom halves $H^b_i$ in pairs and get the new subsets: $\displaystyle \sA^b_k$ except for the last half $H^b_n$.
% \\ Return all the merged front halves $\{\displaystyle \sA^f_1, \displaystyle \sA^f_2,... \displaystyle \sA^f_{(n-1)/2}\}$, all the merged bottom halves $\{\displaystyle \sA^b_1, \displaystyle \sA^b_2,... \displaystyle \sA^b_{(n-1)/2}\}$, the last subset half $H^f_n$ and $H^b_n$. 
% }
% }
% \For{ $l \in 0, 1, ..., logL_S$ }
% {
% \If{$l==0$}
% {
% Initialize the set size: $s$, the list needed to be ranked: $L_S$. \\
% $n = |L_S| / s$, randomly shuffle $L_S$ and divide $L_S$ to $n$ subsets $\displaystyle \sA_i$, where $i\in \{1,2,...,n\}$.
% }
% \Else{
% A\_l, A\_r, H, H = Tree\_Rank($\displaystyle \sA_1, \sA_2,...\sA_n$)
% }
% }
% \end{algorithm}


==> benchmark.tex <==
\section{benchmark}
% \input{figures/overview}

\input{tables/benchmark}
\input{tables/table_stat}

% \textbf{Data Construction}
% Based on TURL's related work beginning to revise the summary paragraph.

% do we evaluate the different aspects? for example, the table interpretation mainly needs to understand the special information of columns, last three tasks need global reasoning?

% Give footnote on the table to clarify the definition of pos and neg

% how we get the detailed dataset for each task. And we make sure that the training set and the eval set don't overlap. Where are the candidates come from? For both training and test?

% We evaluate LLMs on table understanding from different perspectives: organize this (very important, to show different data/tasks verify which aspect?) 
To construct our benchmark, we consider four scenarios that widely show up in the real world: (1) Can LLMs extract knowledge from tables? (2) Can LLMs assist users during operating tables? (3) Can LLMs directly answer questions based on tables? (4) Can LLMs verify table facts and discriminate claims? We construct the instruction tuning dataset to empower LLMs to complete table tasks in these four scenarios.

\subsection{Table Interpretation.}

Table interpretation aims to uncover the semantic attributes of the data contained in the tables and extract the knowledge from tables (Figure\ref{fig:overview}). Column type annotation, relation extraction and entity linking are crucial tasks for table interpretation and fundamental steps for many downstream tasks like data integration and knowledge discovery\citep{?}. Based on the labeled column types, labeled relations between column pairs and linked entities, the table data can be used to construct knowledge bases ($KB$).
% Given the model a table, the model needs to understand what is the column about and label the column with correct types. The model needs to understand the relation between two columns and label the column pairs with correct relations. In order to link an entity of a table to a correct entity in Wikidata, the model needs to understand what the table is about and what the entity refers to. 
These three tasks involve the common procedure that the model needs to make choices from given candidates, thus we formulate these three tasks as the classification tasks (multi-choice QA). Column type annotation and relation extraction are multi-label classification problems where candidate sizes (i.e., the entire categories: column types and relation types respectively) are fixed and the same for all tables. For entity linking, there is only one ground truth so it's a single-label classification problem, but the ground truth is different based on the table and entity. The candidates for each entity are the retrieved entities by the Wikidata Lookup service, and the candidate size for each entity varies.
% Column type annotation is a crucial task for table understanding and is a fundamental step for many downstream tasks like data integration and knowledge discovery. \citep{?} 
% Most existing work [29, 35, 48] assumes that all relations between entities are known in KB and relations between columns can be easily inferred based on entity linking results. However, such methods rely on entity linking performance and suffer from
% KB incompleteness. Here we aim to conduct relation extraction without explicitly linking table cells to entities. This is important as it allows the extraction of new knowledge from Web tables for tasks like knowledge base population.
% Entity linking is usually addressed in two steps: a candidate generation module first proposes a set of potential entities, and an entity disambiguation module then ranks and selects the entity that best matches the surface form and is most consistent with the table
% context. Following existing work [4, 16, 35], we focus on entity disambiguation and use an existing Wikidata Lookup service for candidate generation.


\noindent \textbf{Column Type Annotation.} Given a table $T$ and a set of semantic types $\mathcal{L}$, column type annotation aims to annotate a column in $T$ with $l\in\mathcal{L}$ so that all entities in the column have type $l$. In our dataset, a column can have multiple types, so we formulate it as a multi-label classification problem. In our formulation, we randomly select an entity from the target column and explicitly ask the model to choose the correct types from the entire categories for it. Our dataset contains 255 column types in total from Freebase \citep{} due to its richness, diversity and scale. The column types are present in a long-tailed distribution.



\noindent \textbf{Relation Extraction.} Given a table $T$ and a set of relations $\mathcal{R}$ in $KB$. For a subject-object column pair in $T$, we aim to annotate it with $r\in\mathcal{R}$ so that all entity pairs in the columns have the same $r$. The subject column is the first column while the object column is one of the rest in the table. In our dataset, a subject-object column pair can own multiple relations, which is a multi-label classification problem as well. In our formulation, we randomly select an entity pair and explicitly ask the model to choose the correct relation types from the given relation categories. Our dataset contains 121 relation types in total from Freebase and the relation types are in a long-tailed distribution.

% associate a pair of columns in a table with the KB relation that holds between each pair of entities in a given row of the columns
% Data statistics (long tail graph)

\noindent \textbf{Entity Linking.} Given a table $T$ and a knowledge base $\mathcal{KB}$, entity linking aims to link each potential entity mention in cells of $T$ to its referent entity $e\in\mathcal{KB}$. For Wikipedia tables, each table contains multiple entity mentions in cells and each entity mention can be associated with a referent entity in Wikidata. We use Wikidata Lookup service to retrieve the referent entities as candidates for each entity mention and let LLMs choose the correct referent entity from the retrieved candidates.

\subsection{Table Augmentation.} 
Table augmentation refers to the task that expands a seed query table with additional data (Figure\ref{fig:overview}). Imagine a scenario where there is a user working with a table at some intermediate stage and has already set the table caption and entered some data into the table. The table is assumed to have column headers (i.e., column names) that are located above the first content row to identify each column. Table augmentation aims to provide users “smart suggestions,” that is, recommending (i) additional entities (row population) and (ii) additional column headers (schema augmentation).
We follow [45, TURL] to formulate these two tasks as ranking problems. 
% The candidate size for row population training, schema augmentation training and inference are limited, but the candidate size for row population is very large and can range from ? to ?. 


\noindent \textbf{Row Population.} Given a partial table $T$, and a seed subject entity, row population aims to generate more entities to fill the subject column. The subject column is the first column in the table. The subject entity is the cell at the intersection of the first content row and the first column. We use KNN to retrieve 10 most similar tables from the existing training corpus \citep{} for each table and collect their subject entities. We rank the retrieved subject entities based on their table similarity and use the ranked entities to construct the instruction tuning dataset for training. During inference, we follow [45, TURL] to use their candidate generation module, which formulates a search query using either the table caption or seed entities and then retrieves tables via the BM25 retrieval algorithm. Subject entities in those retrieved tables are the candidates for evaluation. 


\noindent \textbf{Schema Augmentation.} Given a partial table $T$ that has a caption and a seed header, and a header vocabulary $\mathcal{H}$, schema augmentation aims to recommend a ranked list of headers $h\in\mathcal{H}$ to add to $T$. We use KNN to retrieve 10 most similar tables from the existing training corpus and inference corpus \citep{} for each table and collect their headers for training and evaluation respectively. We rank the retrieved headers based on their table similarity for training and let LLMs rank the retrieved headers during inference. 

\subsection{Question Answering.}
Table question answering requires models to identify multiple discontinuous facts in the tables and do reasoning and integration of those facts to generate correct answers. As LLMs have demonstrated strong ability to answer human questions, we include two existing complex table question answering datasets to evaluate the capability of LLMs.

\noindent \textbf{Free-form QA (FeTaQA) \citep{}.} Given a table $T$, multiple highlighted cells $C$, a question $Q$, this task is to generate the answer based on $C$. The answers in FeTaQA are human-generated explanations involving entities and their high-level relations present in the free form.

% Existing table question answering datasets
% contain abundant factual questions that primarily evaluate the query and schema comprehension capability of a system, but they fail to include questions that require complex reasoning and integration of information due to the constraint of the associated short-form answers. To address these issues and to demonstrate the full challenge of
% table question answering, we introduce FeTaQA, a new dataset with 10K Wikipediabased {table, question, free-form answer, supporting table cells} pairs. FeTaQA yields a more challenging table question answering setting because it requires generating free-form text answers after retrieval, inference, and integration of multiple discontinuous facts from a structured knowledge source. Unlike datasets of generative QA over text in which answers are prevalent with copies of short text spans from the source, answers in our dataset are human-generated explanations involving entities and their high-level relations.

\noindent \textbf{Hierarchical Table QA (HiTab \citep{}).}
 HiTab is constructed from a wealth of statistical reports and Wikipedia pages, which nearly all tables are hierarchical and include complex numerical reasoning. The questions are revised from real and meaningful sentences authored by analysts.

\subsection{Fact Verification.}
\noindent \textbf{TabFact.} Given a table $T$, a statement $s$, fact verification is to discriminate whether $s$ is entailed or refuted based on $T$ as the evidence. The statements are all human-annotated natural language statements. Table fact verification is challenging as it involves both soft linguistic reasoning and hard symbolic reasoning.

% TabFact involves 16k Wikipedia tables as the evidence for 118k human-annotated natural language statements, which are labeled as either ENTAILED or REFUTED. TabFact is challenging since it involves both soft linguistic reasoning and hard symbolic
% reasoning. 

\subsection{Data Statistics.}

For table interpretation and table augmentation, we follow TURL to get the initial training and evaluation corpus, which are created based on the original WikiTables corpus\citep{}. As the data size is very large, we do sampling from the raw data corpus. Data statistics are shown in table\ref{tb:table_stat}

For training data construction, we randomly sample 20k tables for column type annotation, relation extraction and fact verification. For entity linking, as one table contains many entities, we sample 2k tables. We sample 30k tables for schema augmentation. For Hitab and Fetaqa we include their full train data due to their small size. For row population, we randomly sample 20k tables and filter out tables that have no more than 3 rows, and finally get 15056 tables. For column type annotation, relation extraction and entity linking, as they are classification tasks and the candidates are large, we split them into smaller sets. We add a "none of the above" option for each set. The categories in each set are given in the instruction for models to make the choice. `Pos' refers to the instances that true labels are in the candidates of the instruction and the ground truth is the true labels. `Neg' refers to the instances that ground truth is the "none of the above" option. For all datasets we used, there are no overlaps between the training set and the evaluation set.

==> experiments.tex <==
\section{Experiments}
% \input{tables/llm}

\nop{\hs{do we still want to put the results of models from earlier experiments where you use the tricks to deal with long contexts? If so, you should think about how to describe them in the main content without diving into too many details. I think you might just include Llama 2's results there, i.e, there are llama 2 (with short pruned candiates using your tricks) vs Llama 2 (with long context using LongLoRa).}}

We demonstrate the capability of completing table tasks on five LLMs: Alpaca, Llama-2, Llama-2-Chat, Vicuna-1.5, and Tulu. Alpaca is an instruction-tuned model that originates from Llama-1. Llama2 is a more powerful pretrained model, which has demonstrated better performance than Llama-1. Llama-2-Chat is a fine-tuned version of Llama-2 that is optimized for dialogue use cases. It's trained by alignment techniques such as instruction tuning and RLHF. Vicuna-1.5 is the latest version by fine-tuning Llama 2 on user-shared conversations collected from ShareGPT. Tulu is a Llama model finetuned on a mixture of instruction datasets such as FLAN V2, CoT, Dolly, Open Assistant 1, GPT4-Alpaca, Code-Alpaca, and ShareGPT. These are LLaMA families with only the decoder architecture. Due to the computing resource limit, we only evaluate the performance of the 7B model for the LLaMA family and leave the larger size model performance for future work. We also largely reduce the training examples, which are 100 training examples and 1000 training examples for each task to demonstrate LLMs' ability.


% In addition, we also try Flan-T5, which has a comparable model size but has an encoder-decoder architecture.
 % For Flan-T5, we try 3B or 11B???
% show a large table contain eight tasks, each with a number (representative metric). For full metric table, put it in appendix.

\noindent\textbf{Evaluation Metrics.}
We follow existing work to use their metrics. For multi-label classification tasks (column type annotation and relation extraction), we use precision, recall and F1. For entity linking which there is only one ground truth and fact verification, we use accuracy. For ranking tasks (row population and schema augmentation), we use MAP (mean average precision). For free-form QA, we use scareBLEU, Rough-1, Rough-2, Rough-L and METEOR. For hierarchical table QA, we use execution accuracy.


\noindent\textbf{Training and Inference Details.}
For the dynamic table segmentation, the reserved instruction length for free-form QA is 50; for entity linking is 500; for other datasets is 100. The offset for all tasks is 200. The reserved table metadata length for all tasks is 20. We train LLaMA-family models for 1 epoch when using the entire 968k training data. We train 3 epochs when using 100 and 1000 training examples. The candidate size in the instructions for column type annotation, relation extraction and entity linking is 10,
The subset size for row population is 20.
The max generation length for row population is 512; for free-form QA and schema augmentation is 128; for others is 64. 


==> guidelines.tex <==
\section{Submission of conference papers to ICLR 2024}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2024 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2024_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2024_conference.sty+ and \verb+iclr2024_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2024_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


\bibliography{iclr2024_conference}
\bibliographystyle{iclr2024_conference}

\appendix
\section{Appendix}
You may include other additional sections here.




==> intro-v2.tex <==
\section{Introduction}

% Table tasks are important.

% LLM is fastly development. Unified model is a trend. Assistance human

% There lacks a comprehensive benchmark to evaluate LLM performance on table tasks.

% why instruction-tuning? 

 % various document types and database systems such as webpages, spreadsheets, PDFs, and MySQL. As a ubiquitous semi-structured format, tables are widely used in  This ubiquity has drawn the keen interest of the research community, leading to a surge in efforts aimed at designing models for handling various table tasks. 

Tables have emerged as indispensable data structures to store and present information in various domains, spanning from scientific research, business reports, healthcare records to financial statements. In this work, we seek to answer the question: \textit{Can we build a generalist model that can excellently handle different table tasks?} A generalist model for tables could make the tables more easily to be manipulated and annotated, thus can serve as a user-friendly tool to largely reduce manual labor \citep{}.

A generalist model for tables shall meet the following desiderata: First, \textbf{it shall work on diverse table tasks.} XX Second, \textbf{it shall work on real-world tables, which can be large, complex, and incomplete.}
% With the advanced development of neural models for different applications such as vision(), language(), different model architecture designs () and pretraining methods() have been proposed to aid table understanding and have achieved remarkable progress recently. 

Building models for tables is not new. There have been numerous prior efforts in varied forms. However, none of them meets all the requirements for a generalist model listed above. Existing work falls short in one to all of the following aspects: 1) Requires table pretraining and/or special model architecture design for tables \citep{}, 2) only supports a limited specific type of tables and tasks \citep{}, (3) making strong simplifying assumptions about tables \citep{}. Meanwhile, LLMs have been shown to excel at grounded language understanding in structured knowledge \citep{}. It's therefore promising to explore LLMs as a candidate solution towards generalist models for tables. However, there lacks a comprehensive dataset and task collection that can support the development and evaluation of generalist table models, which is one of the focus of this work.

In light of this, we construct \texttt{TableBench}, a new table-specific dataset with diverse table tasks. As instruction tuning has shown its effectiveness in guiding LLMs to better follow instructions to complete tasks, we specially design the instructions for each task. In summary, \texttt{TableBench} offers the following unique features:

\textbf{1.Diverse coverage of tasks.} \texttt{TableBench} collects 8 tasks that are widely used 
\textbf{2.Use of real-world tables.}



% Recently, large language models (LLMs) such as ChatGPT, PaLM and Llama family have exhibited notable power in language understanding and generation. Such large language models have shown their amazing intelligence in completing various tasks such as summarization and question answering, which can effectively communicate with humans and be treated as powerful human assistants to provide different services. Therefore, empowering LLMs with table understanding ability is very important, which can not only leverage the existing language understanding ability and knowledge, but also provide a convenient unified interface to assist users handling table tasks.




% Thus, we are curious whether we can enable large language models to gain the ability to understand and effectively handle table-related tasks. As it can be a crucial advancement which holds significant implications for enhancing information extraction, decision-making and knowledge integration. Moreover, the integration of table understanding into language models enables more sophisticated human-machine interactions. 


 % As instruction tuning has shown its effectiveness in guiding LLMs to better follow instructions to complete tasks, we adapt instruction tuning to study the following question: \textit{can LLMs excellently handle different table tasks by following instructions?} Towards this end, we propose a comprehensive table benchmark (\texttt{TableBench}) that unifies different table types and different table tasks that widely appear in four scenarios: (1) extract knowledge from tables; (2) assist users when operating tables; (3) communicate with humans to answer table-related questions; (4) verify table facts and discriminate the claims. We construct 968k table-specific instruction tuning dataset to explore the table understanding capability of the instruction-following LLMs. 

\input{figures/overview}
As we explore real-world tables which often contain large tables, and some table classification and ranking tasks contain large categories and candidates respectively, which exceed the maximum input length limit of LLMs, we propose three algorithms: dynamic subtable segmentation, divide-and-merge and tree-rank to resolve them respectively. Dynamic subtable segmentation reserves different lengths for different components of instructions for different tasks and calculates the allowed subtable length and segments table accordingly. Divide-and-merge first divides entire large categories into different subsets and each subset is formulated as the candidates in a multi-choice QA problem for models to make the choice, then merges the answer from all the subsets. Tree-rank ranks entire candidates by multiple node splitting and merging processes, which prioritizes merging the top-ranked half node pairs each time. Our experiments show that: with only no more than 1.4\% training data, LLMs can achieve more than 60\% SOTA performance on most table tasks; with 5\%-40\% training data, LLMs can achieve more than 80\% SOTA performance on most table tasks, and some can even be better than SOTA.

In summary, we highlight our contributions from two perspectives: (1) From the data engineering perspective, we present \texttt{TableBench}, which introduces different table types and table tasks from four popular human-machine interaction scenarios and construct 968k table-specific instruction tuning dataset accordingly. These tasks have dissimilar characteristics which need special instruction design for each task. (2) From the methodology perspective, we propose three algorithms: dynamic subtable segmentation, divide-and-merge and tree-rank to address three challenges: large table input, large category classification and large candidate ranking caused by the limited table input length constraints of LLMs. (Should we hightlight our contributions like this?)





% In addition, various table-related tasks have been proposed to leverage models to automatically test the different aspects understand tables. For example, column type annotation, table augmentation. xxx which uses to assist human table interaction. [46]in Xiang's paper.

% As large language models such as ChatGPT, XX has demonstrated XX power that can have fantastic conversations with humans, they can understand human intent well and handle different tasks such as XX. In this work, we propose to see whether large language models are strong table representers that without special model design for table pretraining and also without large table-based corpus for table pretraining, whether existing large language models have strong ability to handle table tasks.




 

% We formulate the instruction? how? how to mention large candidates for several differnt type of tasks? how to mention ranking?

% During the development of our instruction-following model, there are two main challenges due to the constrained context length (?): (1)Candidates Iteration (2) Ranking Formulation

% LLM is important and unified to solve all, so as for table tasks.



==> intro.tex <==
\section{Introduction}

% Table tasks are important.

% LLM is fastly development. Unified model is a trend. Assistance human

% There lacks a comprehensive benchmark to evaluate LLM performance on table tasks.

% why instruction-tuning? 

Tables have emerged as indispensable data structures to store and present information in various document types and database systems such as webpages, spreadsheets, PDFs, and MySQL. As a ubiquitous semi-structured format, tables are widely used in various domains, spanning from scientific research, business reports, healthcare records to financial statements. This ubiquity has drawn the keen interest of the research community, leading to a surge in efforts aimed at enhancing table comprehension. 

% With the advanced development of neural models for different applications such as vision(), language(), different model architecture designs () and pretraining methods() have been proposed to aid table understanding and have achieved remarkable progress recently. 

Recently, large language models (LLMs) such as ChatGPT, PaLM and Llama family have exhibited notable power in language understanding and generation. Such large language models have shown their amazing intelligence in completing various tasks such as summarization and question answering, which can effectively communicate with humans and be treated as powerful human assistants to provide different services. Therefore, empowering LLMs with table understanding ability is very important, which can not only leverage the existing language understanding ability and knowledge, but also provide a convenient unified interface to assist users handling table tasks.

% Thus, we are curious whether we can enable large language models to gain the ability to understand and effectively handle table-related tasks. As it can be a crucial advancement which holds significant implications for enhancing information extraction, decision-making and knowledge integration. Moreover, the integration of table understanding into language models enables more sophisticated human-machine interactions. 


 As instruction tuning has shown its effectiveness in guiding LLMs to better follow instructions to complete tasks, we adapt instruction tuning to study the following question: \textit{can LLMs excellently handle different table tasks by following instructions?} Towards this end, we propose a comprehensive table benchmark (\texttt{TableBench}) that unifies different table types and different table tasks that widely appear in four scenarios: (1) extract knowledge from tables; (2) assist users when operating tables; (3) communicate with humans to answer table-related questions; (4) verify table facts and discriminate the claims. We construct 968k table-specific instruction tuning dataset to explore the table understanding capability of the instruction-following LLMs. 

\input{figures/overview}
As we explore real-world tables which often contain large tables, and some table classification and ranking tasks contain large categories and candidates respectively, which exceed the maximum input length limit of LLMs, we propose three algorithms: dynamic subtable segmentation, divide-and-merge and tree-rank to resolve them respectively. Dynamic subtable segmentation reserves different lengths for different components of instructions for different tasks and calculates the allowed subtable length and segments table accordingly. Divide-and-merge first divides entire large categories into different subsets and each subset is formulated as the candidates in a multi-choice QA problem for models to make the choice, then merges the answer from all the subsets. Tree-rank ranks entire candidates by multiple node splitting and merging processes, which prioritizes merging the top-ranked half node pairs each time. Our experiments show that: with only no more than 1.4\% training data, LLMs can achieve more than 60\% SOTA performance on most table tasks; with 5\%-40\% training data, LLMs can achieve more than 80\% SOTA performance on most table tasks, and some can even be better than SOTA.

In summary, we highlight our contributions from two perspectives: (1) From the data engineering perspective, we present \texttt{TableBench}, which introduces different table types and table tasks from four popular human-machine interaction scenarios and construct 968k table-specific instruction tuning dataset accordingly. These tasks have dissimilar characteristics which need special instruction design for each task. (2) From the methodology perspective, we propose three algorithms: dynamic subtable segmentation, divide-and-merge and tree-rank to address three challenges: large table input, large category classification and large candidate ranking caused by the limited table input length constraints of LLMs. (Should we hightlight our contributions like this?)





% In addition, various table-related tasks have been proposed to leverage models to automatically test the different aspects understand tables. For example, column type annotation, table augmentation. xxx which uses to assist human table interaction. [46]in Xiang's paper.

% As large language models such as ChatGPT, XX has demonstrated XX power that can have fantastic conversations with humans, they can understand human intent well and handle different tasks such as XX. In this work, we propose to see whether large language models are strong table representers that without special model design for table pretraining and also without large table-based corpus for table pretraining, whether existing large language models have strong ability to handle table tasks.




 

% We formulate the instruction? how? how to mention large candidates for several differnt type of tasks? how to mention ranking?

% During the development of our instruction-following model, there are two main challenges due to the constrained context length (?): (1)Candidates Iteration (2) Ranking Formulation

% LLM is important and unified to solve all, so as for table tasks.



==> methodology.tex <==
\section{methodology}

In this section, we elaborate on the key challenges and our solutions during the unification of different table tasks. There are three main challenges due to the constrained input length of LLMs: (1) large table input; (2) large category classification; (3) large candidate ranking. We design dynamic subtable segmentation, divide and merge and tree rank algorithms to solve them respectively. 

\noindent \textbf{Dynamic Subtable Selection.} As our tables are from the Web (Wikipedia tables) or scientific reports (spreadsheet tables), they often have varied lengths. Some tables have long contents which will exceed LLMs' input limit. Since different tasks have different table metadata and different instructions and the length for them can vary significantly, we design a dynamic subtable segmentation method to dynamically control the segmented table length for each task. Specifically, we reserve different lengths for different components in the instructions for different tasks, and then calculate the allowed subtable length and truncate the table accordingly. For each table, if the entire input is out of the model input length limit, we will segment the table contents and only maintain the most related subtable (consecutive rows) as the context for models to complete this task. We can get a subtable set through Algorithm\ref{algo1} in Appendix (). We use offset (should we mention offset here as the algorihtm is in Appendix?) to help identify the start position (start row) of each subtable in the raw table. As cutting the table based on the calculated length may cause the row truncated in the middle and the row may be missing after postprocessing, we use offset to add extra rows to each subtable so as to make sure there are overlapped rows among adjacent subtables and there are no rows missing. After we get the subtable set, we use heuristic matching to identify the final subtable. More specifically, for column type annotation, we use the entity in the target column to identify the final subtable. For relation extraction, we use the entity pairs between the target column pairs to match the final subtable. For entity linking, we use entity mention to find the final subtable. For row population and schema augmentation, as we need models to populate the columns/headers, there is no input table thus no subtable needs to be selected. For hierarchical table QA, free-form QA and fact verification, as most tables in these datasets are within length constraints, we directly select the first segmented subtable (which is often the entire table) as the final subtable. 
% there are >80\% ? (double check this) tables within the length limit and also there is global reasoning spanning different columns and rows. We leave how to handle the global reasoning among different subtables as the future work.



\noindent \textbf{Divide and Merge.} For column type annotation and relation extraction, there are more than hundreds of categories (types/relations) for models to select. For entity linking, the category (referent entities with their description) size ranges from ? to ? As we formulate these three tasks as multi-choice QA tasks, and their choice size is large; in addition, the types and relations are from Freebase, and the referent entities with their description are from Wikidata, thus each choice is long which takes up several tokens after tokenization. Therefore, it's difficult for LLMs to choose the correct answer from all the given choices if we put all the choices into the model input at once . \\
To solve this, we design a `divide and merge' method. More specifically, we first divide all choices into multiple subsets, then add a ``none of the above" option to the choices for each subset. If the ground truth labels are not in the candidates, the ground truth will be ``none of the above", otherwise it will be the true labels. There is only a ``divide" procedure for training. During inference, we have the same ``divide" procedure, but we have an extra ``merge" procedure to merge all the predictions and ground truths from all the subsets. Then we remove all the ``none of the above" from both ground truths and predictions to get the final predicted labels for evaluation. The details are shown in Algorithm\ref{algo2}. \\

\noindent \textbf{Tree Rank.} When the model needs to rank a large size of candidates and each candidate
\begin{wrapfigure}[28]{r}{0pt}
\centering
% \flushright
% \begin{center}
%\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[width=0.5\linewidth]{figures/rank_algo.png}
% \end{center}
\caption{Illustration of tree rank.}
\label{fig:rank_algo}
\end{wrapfigure} 
is long. A special design is needed to handle such a case. For example, we follow existing work \citep{} to formulate row population as a ranking problem.  We denote the candidate list as $L_{C}$, the goal is to get the top-k from the final ranked list. We predefine the candidate size in each subset size as $S$. The number of subset is $n = |L_{C}| / S$. We first randomly shuffle $L_C$ and divide $L_C$ to $n$ subsets $\displaystyle \sA_i$, where $i\in \{1,2,...,n\}$. Figure\ref{fig:rank_algo} illustrates the details. First, we divide the entire candidates (size $nS$) into several subsets denoted as $\displaystyle \sA_i$, with each subset size $S$. For the first layer, we let the model rank each subset $\displaystyle \sA_i$. After ranking, each subset will be divided into two nodes, with each node size $S/2$. The red round nodes are the ranked top-half elements, while the blue round nodes are the ranked bottom-half elements. Then we merge all the red round nodes and blue round nodes in pairs to get the second layer. For splitting and merging each time, there will be two sublayers: the left sublayer and the right sublayer derived from this layer/sublayer. If the red round nodes and blue round nodes are odd, there will be a single node that can not be merged in this layer. We convey it to the next layer (the red rectangular node and the blue rectangular node) for the later merge and ranking. As the single red round node and blue round node originate from the same subset, they always appear at the same time. For either the merged node or the single node that comes from the red round nodes, we prioritize them and put them in front of the nodes that come from the blue round nodes, which also means the left sublayer matters more than the right sublayer. For the third layer, we merge the red round node (new divided ranked top-half elements) and the red rectangle node (the divided ranked top-half elements from the layer before the last layer) to get the new full node. Finally, we will rank the new full nodes and append the bottom half directly to the ranked full nodes. \\
\textbf{Analysis:} As in our problem, the target candidate size k is mostly no more than $S$, which means the first ranked subset in the final layer matters most and we only care about the candidates in this subset in general, but we still give a ranked order for the rest of the candidates. During the first step, we randomly shuffle all the candidates and divide them into each subset. Then the target candidates will be equally distributed into all subsets with each subset containing $k/n$ target candidates. If the model can rank the candidates in each subset correctly, then after the first ranking and node splitting, each target should be in the top-ranked half of each subset. So the left sublayer matters more than the right sublayer during each splitting and merging. After we merge each node pair and rank it, we can get a new ranked order of the merged subset. But if there is one half that doesn't get the chance in the last layer to be merged because it's single, we prioritize it and merge it with the new top half node.  The larger the candidate size, the more subsets we have, and the more layers there are. The entire layer size is $logn$. The illustration of other numbers of subsets and the detailed algorithm is in Appendix \ref{}.

% (We put the illustration of other scenarios in Appendix \ref{}, do we need them?)
% (Add all the $\displaystyle \sA_1$ etc to the figure, maybe label them as 1,2,3 for easy referring? also make each layer clear. Or call it full node or sub node?)



\input{algorithms/algo2}




% candidate size, target size, MAP - top 20.


% 3) how to unify different types of tasks? eg: FetaQA?

% 1) how to handle large candidate classification task?

% 2) how to handle large candidate ranking task?


% 4) how to handle large tables - cut table to subtable?


% check tulu and llama2 to see how they describe their methodology.

% Formulations of eight tasks.

% multiple candidates (divide and merge)
% each set, multiple-choice QA

% rank 
% short candidates;
% long candidates (several hundreds)-(tree rank)

% The others: 


% algorithm1: Dynamic Table Cut Algorithm

% algorithm2:Tree Rank, calculate the candidate range, target size. -> affects MAP

% add two figures for describing each algo

% \ref{algo1}
% \ref{algo2}
% \ref{algo3}




% When draw the figure, try to visualize the table augmentation process, for entity linking, also visualize using wikipedia, try to make it like an agent.
% Maybe give each example of each type (table interpretation, verification, augmentation, qa). Draw the figure as an agent. (Try to highlight this as it'll be a strong motivation) (AS FIGURE 1) Add a logo "agent"/ LLM 

==> problem_formulation.tex <==
\section{Problem Formulation}

% \noindent \textbf{Unifying the Format.}
\begin{wrapfigure}[10]{r}{0pt}
% \vspace{-3cm}
\centering
% \flushright
% \begin{center}
%\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[width=0.5\linewidth]{figures/problem_formulation.png}
% \end{center}
\caption{An example of column type annotation.}
\label{fig:format}
\end{wrapfigure}
We format all datasets to follow a chatbot-style schema to unify varied task designs, shown in Figure\ref{fig:format}. The format starts from a prompt as a prologue, followed by the table metadata (Wikipedia page title, Wikipedia section title and table caption) and serialized table headers and contents, then the specific instruction design for each task. For the prompt design, we follow the existing instruction-tuned LLMs' prompts. The detailed instruction design for each task is in Appendix (). 

==> results_analysis.tex <==
\section{Results and Analysis.}
\input{tables/results}
\subsection{Overall Performance.}
Table\ref{tb:results} shows the five instruction-following LLMs' performance on our benchmark. Compared the full training size performance among five LLMs, we find that: 
\textbf{(1) There is not a best model across all the tasks. (2) The performances are pretty similar across different LMs for most tasks except for row population.} As those LLMs are either no instruction tuned or instruction tuned on different datasets, we hypothesize that those different datasets help models gain different ability that related to our different tasks, so that in our case, different models are in favor more of different tasks. However, the similar performances indicate those learned ability doesn't significantly matter for most tasks, since Llama-2 is only pretrained without any instruction tuning, but other LLMs' performances are not significantly better than Llama-2. \textbf{(3) With only no more than 1.4\% training data, LLMs can achieve more than 60\% SOTA performance on most tasks; with 5\%-40\% training data, LLMs can achieve more than 80\% SOTA performance, some can even be better than SOTA. }

\subsection{Analysis of different tasks.}

\noindent\textbf{Column Type Annotation.} 
We investigated different factors that affect LLMs' performance on large category classification tasks. We investigate how the Pos and Neg ratio, instruction order, and adding other tasks affect the column annotation task. We do experiment on four settings: (1) Pos:Neg = 1:3, first instruction then table input (2) Pos:Neg = 1:10, first table input then instruction (3) Pos:Neg = 1:3, first instruction then table input (4) Pos:Neg = 1:3, unified model, first instruction then table input. 
\begin{wraptable}[11]{r}{5cm}
% \vspace{-0.5cm}
\centering
\caption{Column Type Annotation: controllable experiments on Alpaca.}
\begin{tabular}{l|ccc}
\toprule
 & Precision & Recall & F1  \\
\midrule
(1) & 81.60 & 85.08 & 83.30 \\
(2) & 88.49 & 87.55 & 88.02 \\
(3) & 81.17 & 92.58 & 86.50 \\
(4) & 81.36 & 92.14 & 86.41\\
\bottomrule
\end{tabular}
\end{wraptable}

Comparing (1) with (2), we can see the ratio of the positive class and the negative class matters: both precision and recall improve largely by increasing the negative class training examples. Comparing (1) with (3), we can see the order of the instruction and the table matters: the precision improves largely while precision is maintained. As \citep{liu2023lost} finds that LLMs' performance is always highest when the relevant information occurs at the beginning or the end of the input context, our observation may be because the candidates are at the end of the instruction and the model will pay more attention to the candidates so as to help models choose more correct candidates easily.  Comparing (1) and (4), we can see merging other table tasks matters, which can increase the recall largely for the column type annotation task.

% The class is in long-tailed distribution, but we don't see the precision, recall, and F1 of each column type have a strong correlation with the long-tailed distribution. (maybe put the distribution figure for both few-shot and full settings? few-shot may be more interesting to see the generalization ability as the training examples are very small)

\noindent\textbf{Entity Linking.}
We observe most of the errors come from the model choosing a very similar entity name while the description is not correct. Since the description is usually highly correlated with the Wikipedia page title, we hypothesize that the model doesn't get enough attention on the title so choose the wrong entity. This indicates for the instruction design, giving some special hints to explicitly highlight the Wikipedia title may help the model make the correct choice.

\noindent \textbf{Table QA and Fact Verification.}
In our experiments (Figure\ref{tb:hitab_transfer}, we found that after unifying 
\begin{wraptable}[14]{r}{8cm}
\vspace{-0.4cm}
\centering
\caption{Performance of task transfer on Alpaca. `Unified' means training a unified model with merged data from eight tasks.}
\begin{tabular}{lccccc}
\toprule
Train & \multicolumn{2}{c}{} & Hitab & Unified \\
\midrule
\multirow{7}{*}{Eval}&{Hitab} & Exec Acc & \textbf{58.71} & 34.47  \\
\cmidrule(lr){2-5}
& \multirow{5}{*}{FeTaQA} & sacreBLEU & 23.47& \textbf{36.62}  \\
 &  & Rough-1 & 19.70 & \textbf{71.11} \\
 &  & Rough-1 & 9.23 & \textbf{48.43} \\
 &  & Rough-L & 18.14 & \textbf{59.82}  \\
 & & METEOR & 8.84 & \textbf{63.55}  \\
\cmidrule(lr){2-5}
& TabFact & Accuracy &15.42 & \textbf{66.93}   \\
\bottomrule
\end{tabular}
\label{tb:hitab_transfer}
\end{wraptable}
 different tasks to get one unified model, the performance drops significantly for hierarchical table QA (Hitab) task compared with only instruction tune the single task. As (Gudibande et al., 2023) proposed that instruction tuning mainly improves on tasks that are heavily supported in its training dataset, we hypothesize that the performance drop is due to the very smaller training size for hierarchical table QA task, if compared with other tasks when training a unified model. In addition, we also show the performance on task transfer among Hitab, FeTaQA and TabFact. We can see if the model is only instruction tuned on Hitab, then the model performance for FeTaQA and TabFact will have a large gap compared with the unified model, which also demonstrates the necessity of constructing table-specific data from different tasks and training the generalist models for tables.
% we hypothesize that this is because Hitab contains complex hierarchical spreadsheets while other tasks are all Wikipedia tables. So the unified instruction tuning mainly learn the structure of the Wikitable but not spreadsheet which leads to worse performance of Hitab. It also indicates how to balance the mixture of different tasks worth further work to pursue. In addition, the FeTaQA explicitly mention the highlighted cells which makes the answer generation easier. However, for hitab and tabfact, the reasoning considers different cells of different columns and rows. When merging other datasets, the model may be disturbed to not learn some reasoning patterns of the single model, so the accuracy for TabFact slightly drops.

% ; (Kung and Peng, 2023) mention that instruction tuning might only capture surface-level patterns and styles
% (e.g., the output format) rather than comprehending and learning the task. 

% \textbf{What tasks are LLMs good at? If not, why? If good, why\\
% All LLaMa-family the results for all the tasks are similar except for XX. How about Flan-T5, which indicates XX is important. Diversity for special table tasks}

% each task, give the analysis of LLM behavior, error type, stat, error reasons. eg: long-tailed entity? none of the above? hullication? tree rank: why


% rank: tree rank results, (add another metric: top 20 include target), phenomenon: not follow instructions, repeated generations, some hallucination, while only 9\% of the target has more than 20 entities (actually there is an assumption: k << S. Give the distribution here.

% 1) algorithm itself; 2) model ranking ability.

\noindent\textbf{Row Population.}
Figure\ref{fig:rank_example} shows an case study for row population task. The left subfigrue shows the initial candidate list which is waiting to be ranked. The orange candidates are target candidates, but currently they scattered in the different places of the entire candidate list. The entire candidate size is around 200. The right subfigure shows the ranked list after applying our tree-rank algorithm. We can see the target candidates are ranked top in the list, which demonstrates the effectiveness of our designed algorithm.


\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[width=\linewidth]{figures/ranking_example.png}
\end{center}
\caption{Sample figure caption.}
\label{fig:rank_example}
\end{figure}

==> tables/backup_main2.tex <==

\begin{table*}[]
\small
\centering
\begin{tabular}{@{}llcclcr@{}}
\toprule
 & Metric & Base & TableLlama & \qquad \qquad SOTA & $\Delta_{Base}$ & $\Delta_{Sota}$ \\ \midrule
\multicolumn{6}{c}{In-domain} \\
\midrule
\multirow{3}{*}{Column Type Annotation} & Precision &  0.00
 & 94.46 & 95.15*\dag~\citep{deng2020turl} & 
 +94.46 & \cellcolor{blue!10}-0.69 \\ 
 & Recall & 0.00 & 94.32 & 93.94*\dag~\citep{deng2020turl} &  +94.32 & \cellcolor{blue!13}+0.38 \\
 & F1 & 0.00 & 94.39 & 94.54*\dag~\citep{deng2020turl} &  +94.39& \cellcolor{blue!11}-0.15\\
\cmidrule(lr){0-6}
\multirow{3}{*}{Relation Extraction} & Precision & 0.00 & 93.09 & 94.57*\dag~\citep{deng2020turl} &  +93.09& \cellcolor{blue!8}-1.48 \\ 
& Recall & 0.00 & 90.83 & 95.25*\dag~\citep{deng2020turl} &  +90.83& \cellcolor{blue!7}-4.42\\
& F1 & 0.00 & 91.95 & 94.91*\dag~\citep{deng2020turl} &  +91.95& \cellcolor{blue!7}-2.96\\
\cmidrule(lr){0-6}
Entity Linking & Accuracy & 0.00 & 93.65 & 84.90*\dag~\citep{deng2020turl} & +93.65& \cellcolor{blue!20}+8.75 \\ 
Schema Augmentation & MAP & 17,27 & 80.50 & 77.55*\dag~\citep{deng2020turl} & +63.23& \cellcolor{blue!15}+2.95 \\ 
Row Population & MAP & 2.83 & 58.44 & 73.31*\dag~\citep{deng2020turl} &  +55.61 & \cellcolor{blue!6}-14.87 \\ 
HiTab & Exec Acc & \text{--} & 64.71 & 47.00*\dag~\citep{cheng2021fortap} &  \text{--}& \cellcolor{blue!25}+17.71\\
FeTaQA & BLEU & 9.47 & 39.05 & 33.44\S~~~\citep{UnifiedSKG} &  +29.58& \cellcolor{blue!18}+5.61\\ 

TabFact & Accuracy & \text{--} & 82.55 & 84.87*~~~\citep{zhao-yang-2022-table}&  \text{--} & \cellcolor{blue!9}-2.32\\ 

\bottomrule
\end{tabular}
\caption{"Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining; "\S": results come from T5-3B. For column type annotation and entity linking, we uniformly sample a subset from the original test data as our test set due to the large test size. For row population, we filter out the examples with more than 500 candidate entities from the original test set and randomly sample a subset as our test set. For all the downsampled test set, we reproduce the SOTA results using the SOTA model. The depth of the color indicates how better our model \texttt{TableLlama} performs compared with the SOTA or base model.}
\label{tab:main_results}
\end{table*}



\begin{table*}[]
\small
\centering
\begin{tabular}{@{}llcclc@{}}
\toprule
 & Metric & Base & TableLlama & \qquad \qquad SOTA & $\Delta_{Base}$  \\
 \midrule
\multicolumn{6}{c}{Out-of-domain} \\
\midrule
FEVEROUS & Accuracy & 37.18 & 72.25 & 82.40\S~~~\citep{UnifiedSKG} & \cellcolor{blue!30}+35.07 \\
HybridQA & Accuracy & 17.69 & 25.71 & 63.40*~~~\citep{eisenschlos2021mate} & \cellcolor{blue!18}+8.02 \\
KVRET & Micro F1 & 36.28 & 48.73 & 67.80\S~~~\citep{UnifiedSKG} & \cellcolor{blue!23}+12.45 \\
ToTTo & BLEU & 3.73 &20.77 & 48.95\S~~~\citep{UnifiedSKG} & \cellcolor{blue!25}+17.04 \\
WikiSQL & Accuracy & 8.70 & 41.68 & 89.50\dag~~~\citep{liu2022tapex} &\cellcolor{blue!30}+32.98 \\
WikiTQ & Accuracy & 32.39 & 31.63 & 57.50\dag~~~\citep{liu2022tapex} & \cellcolor{blue!9}-0.76 \\
\bottomrule
\end{tabular}
\caption{"Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining; "\S": results come from T5-3B. For column type annotation and entity linking, we uniformly sample a subset from the original test data as our test set due to the large test size. For row population, we filter out the examples with more than 500 candidate entities from the original test set and randomly sample a subset as our test set. For all the downsampled test set, we reproduce the SOTA results using the SOTA model. The depth of the color indicates how better our model \texttt{TableLlama} performs compared with the SOTA or base model.}
\label{tab:main_results}
\end{table*}




==> tables/backup_main_results.tex <==

% \begin{table*}[]
% \small
% \centering
% \begin{tabular}{@{}llccl@{}}
% \toprule
%  & Metric & Base & TableLlama & \qquad \qquad SOTA  \\ 
%  \midrule
% \multicolumn{4}{c}{In-domain} \\
% \midrule
% \multirow{3}{*}{Column Type Annotation} & Precision &  0.00
%  & 94.46 & \textbf{95.15}*\dag~\citep{deng2020turl}  \\ 
%  & Recall & 0.00 & \textbf{94.32} & 93.94*\dag~\citep{deng2020turl}  \\
%  & F1 & 0.00 & 94.39 & \textbf{94.54}*\dag~\citep{deng2020turl} \\
% \cmidrule(lr){0-4}
% \multirow{3}{*}{Relation Extraction} & Precision & 0.00 & 93.09 & \textbf{94.57}*\dag~\citep{deng2020turl}  \\ 
% & Recall & 0.00 & 90.83 & \textbf{95.25}*\dag~\citep{deng2020turl} \\
% & F1 & 0.00 & 91.95 & \textbf{94.91}*\dag~\citep{deng2020turl} \\
% \cmidrule(lr){0-4}
% Entity Linking & Accuracy & 0.00 & \textbf{93.65} & 84.90*\dag~\citep{deng2020turl} \\ 
% Schema Augmentation & MAP & 17,27 & \textbf{80.50} & 77.55*\dag~\citep{deng2020turl} \\ 
% Row Population & MAP & 2.83 & 58.44 & \textbf{73.31}*\dag~\citep{deng2020turl}  \\ 
% HiTab & Exec Acc & \text{--} & \textbf{64.71} & 47.00*\dag~\citep{cheng2021fortap} \\
% FeTaQA & BLEU & 9.47 & \textbf{39.05} & 33.44\S~~~\citep{UnifiedSKG} \\ 

% TabFact & Accuracy & \text{--} & 82.55 & \textbf{84.87}*~~~\citep{zhao-yang-2022-table}\\ 

% \bottomrule
% \end{tabular}
% \caption{"Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining; "\S": results come from T5-3B. For column type annotation and entity linking, we uniformly sample a subset from the original test data as our test set due to the large test size. For row population, we filter out the examples with more than 500 candidate entities from the original test set and randomly sample a subset as our test set. For all the downsampled test set, we reproduce the SOTA results using the SOTA model. The depth of the color indicates how better our model \texttt{TableLlama} performs compared with the SOTA or base model.}
% \label{tab:main_results}
% \end{table*}


\begin{table*}[]
\small
\centering
\begin{tabular}{@{}llccl@{}}
\toprule
 & Metric & Base & TableLlama & \qquad \qquad SOTA  \\ 
 \midrule
\multicolumn{5}{c}{In-domain} \\
\midrule
Column Type Annotation &  F1 & 0.00 & 94.39 & \textbf{94.54}*\dag~\citep{deng2020turl} \\
Relation Extraction & F1 & 0.00 & 91.95 & \textbf{94.91}*\dag~\citep{deng2020turl} \\
Entity Linking & Accuracy & 0.00 & \textbf{93.65} & 84.90*\dag~\citep{deng2020turl} \\ 
Schema Augmentation & MAP & 17,27 & \textbf{80.50} & 77.55*\dag~\citep{deng2020turl} \\ 
Row Population & MAP & 2.83 & 58.44 & \textbf{73.31}*\dag~\citep{deng2020turl}  \\ 
HiTab & Exec Acc & \text{--} & \textbf{64.71} & 47.00*\dag~\citep{cheng2021fortap} \\
FeTaQA & BLEU & 9.47 & \textbf{39.05} & 33.44\S~~~\citep{UnifiedSKG} \\ 

TabFact & Accuracy & \text{--} & 82.55 & \textbf{84.87}*~~~\citep{zhao-yang-2022-table}\\ 

\bottomrule
\end{tabular}
\caption{"Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining. For column type annotation and entity linking, we uniformly sample a subset from the original test data as our test set due to the large test size. For row population, we filter out the examples with more than 500 candidate entities from the original test set and randomly sample a subset as our test set. For all the downsampled test set, we reproduce the SOTA results using the SOTA model.  \hs{you should comment a bit on those extremely low numbers like why it achieves zeros.}}
\label{tab:main_results}
\end{table*}



\begin{table*}[]
\small
\centering
\begin{tabular}{@{}llcclc@{}}
\toprule
 & Metric & Base & TableLlama & \qquad \qquad SOTA & $\Delta_{Base}$  \\
 \midrule
\multicolumn{6}{c}{Out-of-domain} \\
\midrule
FEVEROUS & Accuracy & 37.18 & 72.25 & \color{gray}82.40\S~~~\citep{UnifiedSKG} & +35.07 \\
HybridQA & Accuracy & 17.69 & 25.71 & \color{gray}63.40*~~~\citep{eisenschlos2021mate} & +8.02 \\
KVRET & Micro F1 & 36.28 & 48.73 & \color{gray}67.80\S~~~\citep{UnifiedSKG} & +12.45 \\
ToTTo & BLEU & 3.73 &20.77 & \color{gray}48.95\S~~~\citep{UnifiedSKG} & +17.04 \\
WikiSQL & Accuracy & 8.70 & 41.68 & \color{gray}89.50\dag~~~\citep{liu2022tapex} &+32.98 \\
WikiTQ & Accuracy & 32.39 & 31.63 & \color{gray}57.50\dag~~~\citep{liu2022tapex} & -0.76 \\
\bottomrule
\end{tabular}
\caption{"Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining. \zts{The SOTA results come from full-dataset training while the results for \texttt{TableLlama} are zero-shot, so it's unfair to make a direct comparison between them. We put the SOTA results here for reference.} \nop{\hs{can we make the SOTA's number in grey, basically put them here and try not to let people focus on them. you should also point out the SOTA are simply for referrence and it is unfair to make a direct comparison.}}}
\label{tab:main_results}
\end{table*}




==> tables/in_domain_ablation.tex <==
% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{@{}llccccccccc@{}}
% \toprule
% \multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Training \\ Data\end{tabular}} & \multirow{2}{*}{Overall} & ColType & RelExtra & EntLink & ScheAug & RowPop & HiTab & FeTaQA & TabFact \\ \cmidrule(l){4-11} 
%  & &  & F1 & F1 & ACC & MAP & MAP & ACC & BLEU & ACC \\ \midrule
% Base & - &  & - & - & 31.80 & 36.75 & 4.53 & 14.96 & 8.54 &41.65 \\ \midrule
% \multirow{9}{*}{TableLlama} & ColType &  & 94.32 & 0 & 0 & 0 & 0 & 0.13 & 0.52 & 0 \\
%  & RelExtra & & 45.69& 93.96 & 0.45 & 8.72 & 0.99& 7.26 & 1.44 & 0 \\
%  & EntLink & &0.86 & 0.03 & 88.45 & 2.31 & 0.94 &5.37 & 4.79 & 0  \\
%  & ScheAug & - & - & - & - & 80.00 & - & - & - & - \\
%  & RowPop & - & - & - & - & - & 53.86 & - & - & -\\
%  & HiTab & & 0.20 &  & 7.15 & 40.81 & 5.45 & 63.19 & 2.07 & 49.46   \\
%  & FeTaQA &  & 0 &  & 0 & 30.23 & 0.15 & 19.57 & 38.69 & 1.20 \\
%  & TabFact &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74.87 \\ \cmidrule(l){2-11} 
%  & \textbf{TableInstruct} &  & 94.39 & 91.95 & 93.65 & 80.50 & 58.44 & 64.71 &39.05 & 82.55\\ \midrule
% SOTA & & & 94.54 & 94.91 & 84.90 & 77.55 & 73.31 & 47.00 & 33.44 & 84.87 \\ \bottomrule
% \end{tabular}%
% \caption{In-domain test results of the base model, TableLlama and SOTA. }
% \label{tab:my-table}
% \end{table*}


\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Training \\ Data\end{tabular}}  & ColType & RelExtra & EntLink & ScheAug & RowPop & HiTab & FeTaQA & TabFact \\ \cmidrule(l){3-10} 
 &  & F1 & F1 & Acc & MAP & MAP & Acc & BLEU & Acc \\ \midrule
Base &  &  3.01 & 0.96 & 31.80 & 36.75 & 4.53 & 14.96 & 8.54 &41.65 \\ \midrule
\multirow{9}{*}{TableLlama} & ColType &  94.32 & 0 & 0 & 0 & 0 & 0.13 & 0.52 & 0 \\
 & RelExtra & 45.69& 93.96 & 0.45 & 8.72 & 0.99& 7.26 & 1.44 & 0 \\
 & EntLink &0.86 & 0.03 & 88.45 & 2.31 & 0.94 &5.37 & 4.79 & 0  \\
 & ScheAug  & - & - & - & 80.00 & - & - & - & - \\
 & RowPop  & - & - & - & - & 53.86 & - & - & -\\
 & HiTab & 0.20 & 0.14 & 7.15 & 40.81 & 5.45 & 63.19 & 2.07 & 49.46   \\
 & FeTaQA & 0 & 0.40 & 0 & 30.23 & 0.15 & 19.57 & 38.69 & 1.20 \\
 & TabFact & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 74.87 \\ \cmidrule(l){2-10} 
 & \textbf{TableInstruct}   & 94.39 & 91.95 & \textbf{93.65} & \textbf{80.50} & 58.44 & \textbf{64.71} &\textbf{39.05} & 82.55\\ \midrule
SOTA & & \textbf{94.54}*\dag & \textbf{94.91}*\dag & 84.90*\dag & 77.55*\dag & \textbf{73.31}*\dag & 47.00*\dag & 33.44\S & \textbf{84.87}* \\ \bottomrule
\end{tabular}%
\caption{In-domain test results of the base model, TableLlama and SOTA. "Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining. Bold numbers are the best results for each evaluation task. For models trained on the schema augmentation and row population, the predictions on other datasets tend to repeat the candidates in the training data, which means the models cannot generalize to other datasets.}
\label{tab:in_domain_ablation}
\end{table*}

==> tables/llm.tex <==
\begin{table}[h]
\centering
\small
% \scalebox{0.93}{
\begin{tabular}{lcccc}
\toprule
Model & Size & Description \\ \midrule
% \multicolumn{2}{c}{zero-shot} &19.78 & 0 & 15.27 & 4.69 & 9.94 \\ \midrule
Alpaca & 7b & Instruction-tuned model based on LLaMa\\ 
LLaMa2 & 7b & better pretrained model than LLaMa\\ 
Vicuna-v1.5 & 7b & fine-tuning LlaMa 2 from ShareGPT\\ 
Tulu & 7b  & fine-tuned LLaMa on a combination of existing instruction datasets \\
Flan-T5 & 3b/11b & encoder-decoder based; large-scale instruction-tuned model \\
\bottomrule 

Try both full-size and few-shot tuning
% &+ InterCOL(full) & 73.08 & 4.26 & 77.10 & 42.19 & 49.16 \\ \midrule 
\end{tabular}
% }
\caption{LLMs}
\label{llms}
\end{table}



==> tables/main_results.tex <==

\begin{table*}[]
\small
\centering
\begin{tabular}{@{}llcclcr@{}}
\toprule
 & Metric & Base & TableLlama & \qquad \qquad SOTA & $\Delta_{Base}$ & $\Delta_{Sota}$ \\ \midrule
\multicolumn{6}{c}{In-domain} \\
\midrule
\multirow{3}{*}{Column Type Annotation} & Precision &  0.00
 & 94.46 & 95.15*\dag~\citep{deng2020turl} & 
 +94.46 &  -0.69 \\ 
 & Recall & 0.00 & 94.32 & 93.94*\dag~\citep{deng2020turl} &  +94.32 & +0.38 \\
 & F1 & 0.00 & 94.39 & 94.54*\dag~\citep{deng2020turl} &  +94.39& -0.15\\
\cmidrule(lr){0-6}
\multirow{3}{*}{Relation Extraction} & Precision & 0.00 & 93.09 & 94.57*\dag~\citep{deng2020turl} &  +93.09& -1.48 \\ 
& Recall & 0.00 & 90.83 & 95.25*\dag~\citep{deng2020turl} &  +90.83& -4.42\\
& F1 & 0.00 & 91.95 & 94.91*\dag~\citep{deng2020turl} &  +91.95& -2.96\\
\cmidrule(lr){0-6}
Entity Linking & Accuracy & 0.00 & 93.65 & 84.90*\dag~\citep{deng2020turl} & +93.65& +8.75 \\ 
Schema Augmentation & MAP & 17,27 & 80.50 & 77.55*\dag~\citep{deng2020turl} & +63.23& +2.95 \\ 
Row Population & MAP & 2.83 & 58.44 & 73.31*\dag~\citep{deng2020turl} &  +55.61 & -14.87 \\ 
HiTab & Exec Acc & \text{--} & 64.71 & 47.00*\dag~\citep{cheng2021fortap} &  \text{--}& +17.71\\
FeTaQA & BLEU & 9.47 & 39.05 & 33.44~~~\citep{UnifiedSKG} &  +29.58& +5.61\\ 

TabFact & Accuracy & \text{--} & 82.55 & 84.87*~~~\citep{zhao-yang-2022-table}&  \text{--} & -2.32\\ 
\midrule
\multicolumn{6}{c}{Out-of-domain} \\
\midrule
FEVEROUS & Accuracy & 37.18 & 72.25 & 82.40~~~\citep{UnifiedSKG} & +35.07 & -10.15\\
HybridQA & Accuracy & 17.69 & 25.71 & 63.40*~~~\citep{eisenschlos2021mate} & +8.02 & -37.69\\
KVRET & Micro F1 & 36.28 & 48.73 & 67.80~~~\citep{UnifiedSKG} & +12.45 & -19.07\\
ToTTo & BLEU & 3.73 &20.77 & 48.95~~~\citep{UnifiedSKG} & +17.04 & -28.18\\
WikiSQL & Accuracy & 8.70 & 41.68 & 89.50\dag~~~\citep{liu2022tapex} &+32.98 & -47.82\\
WikiTQ & Accuracy & 32.39 & 31.63 & 57.50\dag~~~\citep{liu2022tapex} & -0.76 & -25.87\\
\bottomrule
\end{tabular}
\caption{"Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining. For column type annotation and entity linking, we uniformly sample a subset from the original test data as our test set due to the large test size. For row population, we filter out the examples with more than 500 candidate entities from the original test set and randomly sample a subset as our test set. For all the downsampled test set, we reproduce the SOTA results using the SOTA model. The depth of the color indicates how better our model \texttt{TableLlama} performs compared with the SOTA or base model.}
\label{tab:main_results}
\end{table*}




\begin{table*}[]
\centering
\small
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Training \\ Data\end{tabular}} & \multirow{2}{*}{Overall} & ColType & RelExtra & EntLink & ScheAug & RowPop & HiTab & FeTaQA & TabFact \\ \cmidrule(l){4-11} 
 & &  & F1 & F1 & ACC & MAP & MAP & ACC & BLEU & ACC \\ \midrule
Base & - &  & 0 & 0 & 0 &  17.27 & 2.83 & & 9.47 \\ \midrule
\multirow{9}{*}{TableLlama} & ColType &  & \st{85.03} & 0 & 0 & 0 & 0 &  &  \\
 & RelExtra &  & 45.90 & 92.27 & 0 & 8.7 & 1.04 &  &  \\
 & EntLink & & 0 & 0 & \st{11.75} & 2.3 & 0.01 &  &   \\
 & ScheAug & & 0 & 0 & 0 & 79.80 & 1.1 &  &  &  \\
 & RowPop &  & 0 & 0 & 0 & 34.16 & 53.86 &  &  \\
 & HiTab &  & 0 & 0 & 0 & 40.67 & 5.20 &    \\
 & FeTaQA &  & 0 & 0 & 0 & 16.13 & 0 &  &  \\
 & TabFact &  & 0 & 0 & 0 & 0 & 0 &  &  \\ \cmidrule(l){2-11} 
 & \textbf{TableInstruct} &  & 94.39 & 91.95 & 93.65 & 80.50 & 58.44 & 64.71 &39.05 & 82.55\\ \midrule
SoTA & & & 94.54 & 94.91 & 84.90 & 77.55 & 73.31 & 47.00 & 33.44 & 84.87 \\ \bottomrule
\end{tabular}%
\caption{In-domain test results of the base model, TableLlama and SoTA. }
\label{tab:my-table}
\end{table*}


% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{@{}llccccccc@{}}
% \toprule
% \multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Training \\ Data\end{tabular}} & \multirow{2}{*}{Overall} & FEVEROUS & HybridQA & KVRET & ToTTo & WikiSQL & WikiTQ \\ \cmidrule(l){4-9} 
%  & &  & Acc & Acc & Micro F1 & BLEU & ACC & ACC  \\ \midrule
% Base & - &  &  &  &  &  & \\ 
% \midrule
% \multirow{7}{*}{TableLlama} & ColType &  &  &  &  &  &   \\
%  & RelExtra &  &  &  &  &  &   \\
%  & EntLink &  &  &  &  &  &   \\
%  & ScheAug &  &  &  &  &  &  \\
%  & RowPop &  &  &  &  &  &  \\
%  & HiTab &  &  &  &  &  & \\
%  & FeTaQA &  &  &  &  &  &  \\
%  & TabFact &  &  &  &  &  & \\ \cmidrule(l){2-9} 
%  & \textbf{TableInstruct} &  &  &  &  &  &  \\ \midrule
% SoTA & &  &  &  &  &  &   \\ \bottomrule
% \end{tabular}%
% \caption{Out-of-domain test results of the base model, TableLlama and SoTA. }
% \label{tab:my-table}
% \end{table*}

==> tables/out_domain_ablation.tex <==

\begin{table*}[]
\centering
\small
\begin{tabular}{@{}llccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Training \\ Data\end{tabular}} & \multirow{2}{*}{Overall} & FEVEROUS & HybridQA & KVRET & ToTTo & WikiSQL & WikiTQ \\ \cmidrule(l){4-9} 
 & &  & Acc & Acc & Micro F1 & BLEU & Acc & Acc  \\ \midrule
Base &  & 22.33 & 23.66& 20.72 & 38.90 & 10.39 & 14.84 & 25.48\\ 
\midrule
\multirow{7}{*}{TableLlama} & ColType & 0.28 & 0 & 0 & 0 & 1.11 &0.35 & 0.21   \\
 & RelExtra & 6.44 & 2.38 & 8.17 & 5.90 & 5.60 & 7.02 & 9.58  \\
 & EntLink & 9.06 & 39.04 & 3.06 & 0 & 1.76 & 3.42 & 7.07  \\
 & ScheAug & - & - & - & - & - & - & - \\
 & RowPop & - & - & - & - & - & -  & -\\
 & HiTab & 28.92 & 46.81 & 24.70 & 38.70 & 2.45 & 32.86 & 27.97\\
 & FeTaQA & 25.03 & 1.21 & \textbf{33.79} & \textbf{50.69} & \textbf{23.57} & 13.79 & 27.12 \\
 & TabFact & 9.36 & 56.15 & 0 & 0 & 0 & 0 & 0 \\ \cmidrule(l){2-9} 
 & \textbf{TableInstruct} & \textbf{40.45} & \textbf{72.30} & 27.61 & 48.73 & 20.77 & \textbf{41.68} & \textbf{31.65} \\ 
\cmidrule(l){2-9} 
& $\Delta_{Base}$& \color{blue!70}+18.19& \color{blue!70}+48.64& \color{blue!70}+6.89& \color{blue!70}+9.83& \color{blue!70}+10.38& \color{blue!70}+26.84 & \color{blue!70}+6.15\\
\midrule
SOTA & & \color{gray}68.26 &\color{gray}82.40\S & \color{gray}63.40* & \color{gray}67.80\S & \color{gray}48.95\S & \color{gray}89.50\dag & \color{gray}57.50\dag  \\ \bottomrule
\end{tabular}%
\caption{Out-of-domain test results of the base model, TableLlama and SOTA. "Base": LongLoRA model w/o fine-tuning on \texttt{TableInstruct}; "*": w/ special task-specific model architecture design for tables; "\dag": w/ table pretraining. Bold numbers are the best zero-shot results on each evaluation dataset. The SOTA results come from full-dataset training while the results for \texttt{TableLlama} are zero-shot, so it's unfair to make a direct comparison between them. We put the SOTA results here for reference.}
\label{tab:out_domain_ablation}
\end{table*}

==> tables/results.tex <==


\begin{table*}[h]
\caption{Test set performance of eight tasks under five LLMs. All LLMs' size is 7B. `100' and `1000' refer to training size of each task. `full' refers to the entire training set in our constructed data. The percentage marked as blue refers to the training size ratio compared with the training size used to finetune the SOTA models. The precentage marked as red refers to the performance ratio compared with SOTA. All models are trained in a unified fashion, which we merge the data from all tasks to train the model. The SOTA performance of column type annotation is we reproduced using the SOTA model on our test set. (Remember to cite sota paper)}

\centering
\small
% \scalebox{0.93}{
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule 
\multirow{2}{*}{} & & \multicolumn{3}{c}{Alpaca} & Llama-2 & Vicuna-1.5 & Tulu & Llama-2-Chat & SOTA  \\
 % & & \multicolumn{3}{c}{7B} & 7B & 7B & 7B & 7B & \\
\cmidrule(lr){3-5} \cmidrule(lr){6-9}
\cmidrule(lr){10-10}
& & 100 & 1000 & full &\multicolumn{4}{c}{full}  &  \\
\midrule
\multirow{3}{*}{Column Type Annotation} & Precision & 24.30 & 67.75 ({\color{red}0.08\%x}) ({\color{blue}71\%}) & 88.74 & 89.26 & 88.84 & \textbf{89.48} ({\color{red}5\%x})({\color{blue}94\%}) & & 95.15 \\
& Recall & 30.16 & 64.94 ({\color{red}0.08\%x})({\color{blue}69\%}) & \textbf{87.40} ({\color{red}5\%x}) ({\color{blue}92\%}) & 86.75 & 87.13 & 86.60 &  &94.54 \\ 
& F1 & 26.91 & 66.31({\color{red}0.08\%x})({\color{blue}71\%}) & \textbf{88.07} ({\color{red}5\%x}) ({\color{blue}94\%}) & 87.99 & 87.98 & 88.02 & & 93.94  \\ 
 \midrule 
\multirow{3}{*}{Relation Extraction} & Precision & 32.28 & 59.39 ({\color{red}0.2\%x})({\color{blue}63\%}) & 91.53 & \textbf{93.07} ({\color{red}40\%x})({\color{blue}98\%}) & 92.43 & 92.45 & & 94.57 \\
& Recall & 5.54 & 43.08 ({\color{red}0.2\%x})({\color{blue}45\%}) & \textbf{73.19} ({\color{red}40\%x}) ({\color{blue}77\%}) & 73.00 & 72.14 & 72.28 &  & 95.25  \\ 
& F1 & 9.46 & 49.94 ({\color{red}0.2\%x})({\color{blue}53\%}) & 81.34 & \textbf{81.83} ({\color{red}40\%x}) ({\color{blue}86\%}) & 81.03 & 81.13 & & 94.91  \\ 
\midrule
\multirow{2}{*}{Entity Linking} & EM & 16.69 & 62.57 & \textbf{71.91} & 69.57 & 71.41 & 67.91 & & \text{--} \\
& Relax EM?& 23.34 & 69.73 & 81.77 & \textbf{82.2} & 80.41 & 79.94 &  & \text{--} \\
\midrule
 Schema Augmentation & MAP & 42.06 & 48.84 ({\color{red}0.3\%x})({\color{blue}63\%}) & \textbf{68.10} ({\color{red}10\%x})({\color{blue}88\%}) & 67.74 & 67.39 & 67.89 & & 77.55 \\
 \midrule
 Row Population & MAP & 18.55 & 24.79 & 25.99 & 29.09 & \textbf{53.78} & 45.32 & & \text{--} \\
\midrule
 Hierarchical Table QA & Exec Acc & 30.43 ({\color{blue}68\%}) & 36.74 ({\color{red}14\%x})({\color{blue}81\%}) & 34.47 & \textbf{39.58} ({\color{red}100\%x})({\color{blue}88\%}) & 37.63 & 34.91 & & 45.1 \\
 \midrule
\multirow{5}{*}{Free-form QA} & sacreBLEU & 30.90 ({\color{blue}92\%}) & 35.77 ({\color{red}14\%x})({\color{blue}107\%}) & 36.62 & 36.79 & 36.66 & \textbf{36.93} ({\color{red}100\%x}) ({\color{blue}110\%}) & & 33.44 \\
& Rough-1 & 64.51 ({\color{blue}99\%}) & 69.10 ({\color{red}14\%x})({\color{blue}106\%})  & 71.11 & 71.13 & \textbf{71.32} ({\color{red}100\%x})({\color{blue}109\%}) & 71.27 & & 65.21 \\
& Rough-2 & 41.51 ({\color{blue}96\%}) & 45.87 ({\color{red}14\%x})({\color{blue}106\%}) & 48.43 & 48.56 & \textbf{48.73} ({\color{red}100\%x})({\color{blue}113\%}) & 48.61 & & 43.09 \\
& Rough-L & 53.22 ({\color{blue}96\%})& 57.16 ({\color{red}14\%x})({\color{blue}103\%}) & 59.82 & 59.71 & 59.97 & \textbf{60.20} ({\color{red}100\%x})({\color{blue}109\%}) & & 55.31 \\
& METEOR & 58.64 ({\color{blue}114\%}) & 63.06 ({\color{red}14\%x})({\color{blue}123\%}) & 63.55 & 63.77 & \textbf{63.84} ({\color{red}100\%x})({\color{blue}125\%}) & 63.79 & & 51.23\\
\midrule
Fact Verification & Accuracy& 50.00 & 51.58 ({\color{red}1\%x})({\color{blue}61\%}) & 66.93 & 64.40 & 64.51 & \textbf{68.35} ({\color{red}20\%x})({\color{blue}81\%}) & & 84.2\\
\bottomrule 
\end{tabular}
}
% }
\vspace{-1pc}
\label{tb:results}
\end{table*}




==> tables/table_stat.tex <==


% \begin{table*}[t]
% \caption{Dataset Statistics.}

% \centering
% \small
% % \scalebox{0.93}{
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule 
% \multirow{2}{*}{} & \multicolumn{4}{c}{Train} & \multicolumn{2}{c}{Eval} \\
% \cmidrule(lr){2-5}\cmidrule(lr){6-7}
%  & \# Tables & \# Pos & \# Neg &  \# Training Instances &\# Tables & \# Test Instances 
% \\
% \midrule
% Column Type Annotation  & 20k & 58957 & 600k & 658957 (X columns) & 1k & 71370 (2745 columns)  \\
% Relation Extraction & 20k & 31193 & 150k & 181193 (X column pairs) & 1467 & 26936 (2072 column pairs)  \\ 
% Entity Linking & 2k & 12267 & 36k & 48267 (X entities) & 3350 & 25029 (10k entities) \\ 
% \midrule
% Schema Augmentation & 30k &  \text{--} & \text{--} & 30k & 4646 & 4646 \\
% Row Population & 15056 &  \text{--} & \text{--} & 15056 & 324 & 324\\
% \midrule
% Hierarchical Table QA & 7417 & \text{--} & \text{--} & 7417 & 1584 & 1584 \\
% Free-form QA & 7325 & \text{--} & \text{--} & 7325& 2003 & 2003\\
% \midrule
% Fact Verification & 20k & \text{--} & \text{--} & 20k & 12779 & 12779\\
% \bottomrule 
% \end{tabular}
% }
% \vspace{-1pc}
% \label{tb:table_stat}
% \end{table*}



% \begin{table*}[h]
% \caption{Dataset Statistics of ranking and QA tasks.}

% \centering
% \small
% % \scalebox{0.93}{
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cccc|ccc}
% \toprule 
% Task & \# Training Instances (\# Tables) &  \# Test Instances  (\# Tables)
% \\
% \midrule
% Schema Augmentation & ? & ? \\
% Row Population & ? & ?\\
% \midrule
% Hierarchical Table QA & ? & ? \\
% Free-form QA & ? & ?\\
% \midrule
% Fact Verification & ? & ?\\
% \bottomrule 
% \end{tabular}
% }
% % }
% \vspace{-1pc}
% \label{tb:table_stat_ranking}
% \end{table*}
